Model-based Testing of Mobile Systems -- An Empirical Study on QuizUp Android App

We present an empirical study in which model-based testing (MBT) was applied to a mobile system: the Android client of QuizUp, the largest mobile trivia game in the world. The study shows that traditional MBT approaches based on extended finite-state machines can be used to test a mobile app in an effective and efficient way. Non-trivial defects were detected on a deployed system that has millions of users and was already well tested. The duration of the overall testing effort was of three months, including the construction of the models. Maintaining a single behavioral model for the app was key in order to test it in an efficient way.

==> eptcsdata.tex <==
\providecommand{\firstpage}{16}
\providecommand{\publicationstatus}{L. Aceto, A. Francalanza and A. Ingolfsdottir (Eds.):  Workshop on \\ Pre- and Post-Deployment Verification Techniques (PrePost 2016)\\
EPTCS 208, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.208.2}{10.4204/EPTCS.208.2}}
\pdfoutput=1

